LightSys: Lightweight and Efficient CI System for Improving Integration Speed of Software

The complexity and size increase of software has extended the delay for developers as they wait for code analysis and code merge. With the larger and more complex software, more developers nowadays are developing software with large source code repositories. The tendency for software platforms to immediately update software packages with feature updates and bug-fixes is a significant obstacle. Continuous integration systems may help prevent software flaws during the active development of software packages, even when they are deployed and updated frequently. Herein, we present a portable and modular code review automation system that inspects incoming code changes such as code format and style, performance regression, static analysis, build and deployment tests, and dynamic analysis before merging and changing code. The proposed mechanisms are sufficiently lightweight to be hosted on a regular desktop computer even for numerous developers. The resulting reduced costs allow developers to apply the proposed mechanism to many source code repositories. Experimental results demonstrate that the proposed mechanism drastically reduces overheads and improves usability compared with conventional mechanisms: execution time (6x faster), CPU usage (40% lower), memory consumption (1/180), and no out-of-memory occurrence.

==> note/CI-projects-lists.tex <==


#### Existing CI list (top 10 tools)
https://blog.github.com/2017-11-07-github-welcomes-all-ci-tools/
https://github.com/ciandcd/awesome-ciandcd

https://www.katalon.com/resources-center/blog/ci-cd-tools/ 
(Top 5 CI/CD tools in 2019: Jenkins, CircleCI, TeamCity, Bamboo, GitLab)

Problems with Local platforms (Bamboo, Teamcity and Jenkins, ...)
Problems with Online Platforms (TravisCI, CircleCI, CodeShip, ...)

01. Jenkins,https://jenkins.io/
02. Travis CI,https://travis-ci.org/
03. Circle CI,https://circleci.com/
04. Semaphore CI,https://semaphoreci.com/
05. SWARM CI - https://github.com/ghostsquad/swarmci
06. TeamCity - https://www.jetbrains.com/teamcity/
07. Bamboo -  https://www.atlassian.com/software/bamboo
08. AppVeyor - https://www.appveyor.com/
09. CodeShip - https://codeship.com/
10. Drone - http://try.drone.io/
11. Buildkite - https://buildkite.com/
12. Wercker - http://www.wercker.com/
13. Redhat Tekton - https://github.com/tektoncd/pipeline (apache)
14. Simple CI (Opensource) - https://github.com/lewbor/simpleci
15. Waypoint https://www.waypointproject.io/


#### Youtube Videos


# Webinar: Making CI/CD Builds Faster, sponsored by CircleCI
https://www.youtube.com/watch?v=_Dk6X-S1AJM&ab_channel=TheLinuxFoundation



End of line. 

==> note/survey-code-review-culture.tex <==

* Webpage: http://mosaic.sec.samsung.net/kms/comty.do?comtyId=3292413 (ELV) - survey기능 


코드리뷰문화 조사 - 소스코드의 코드리뷰를 어떻게 진행하고 있으신가요?   
===========================================================================

이제는 당사에서 양산하고 있는 대부분의 디바이스에 운영제체 및 앱플리케이션들이 탑재되고, 소프트웨어의 퀄리티가 제품의 고객 충성도와 고객의 제품 만족도에 직/간접적인 영향을 미치는 시점까지 성큼 왔습니다. 또한, 불과 10년전만 해도 당사 제품의 소프트웨어에는 1인이 개발하여 양산한 소프트웨어들도 많았습니다.  그러나 최근에는 대부분의 소프트웨어를 여러명이서 개발하고 있고, 그 소프트웨어들은 일정 규모이상의 복잡도와 사이즈를 갖게 되었습니다. 

팀프로젝트를 연구 및 개발하기 위하여 동료 개발자들이 작성하는 코드의 리뷰를 얼마나 우리가 유기적으로 소통하며 자발적인 참여를 하고 있을 까요?  본 설문조사는 개발자들이 작성한 소스코드를 병합하기전에 코드리뷰를 어떻게 하고 있는지 공유하고자 합니다. 총 15개의 설문이 있고, 답변을 위해  필요한 예상 소요 시간은 2분 이내입니다. 




1. 현재 당신의 직급이 어떻게 됩니까?

\begin{enumerate}
\item CL1
\item CL2
\item CL3
\item CL4
\item 임원
\item 기타 
\end{enumerate}



2. 현재진행중인 팀프로젝트의 소스코드 관리를 위해 사용하는 Version Control System (VCS)는 무엇인가요?

\begin{enumerate}
\item cvs
\item svn
\item git
\item perforce
\item clearcase
\item 이외  VCS 소프트웨어 
\item 혼자 개발하고 있기 때문에 VCS가 필요 없는 상황이다. 
\end{enumerate}




3. github (또는 gitlab)에서 제공하는 pull request (=merge request)기능을 이용중입니까? 

\begin{enumerate}
\item    예외적인 상황 (개인 프로젝트, 프로젝트 시작 등) 제외하면 거의 PR 사용중이며, 타인의 Approval 없이 Merge되는 일은 거의 없다.
\item    대부분은 PR 사용중이나, 가끔은 공동 프로젝트에서도 Direct Merge하고 있다.
\item   대부분은 PR 사용중이나, Approval 없이 Merge되는 경우 자주 있다.
\item 
\item   PR 거의 사용하지 않는다.
\item   Pull-Request가 아닌 다른 방식의 Code Review/Approval System을 주로 사용한다. (gerrit)
\item 
\item   Pull-Request가 뭔지 모른다.
\end{enumerate}





4. 제출된 pull request의 소스코드에 결함이 있는지 자동으로 점검하는 툴은 무엇입니까?

\begin{enumerate}
\item Jenkins
\item Travis-CI
\item Circle-CI
\item Cirrus-CI
\item Kernel-CI
\item TAOS-CI
\item Azure-Pipeline
\item Semaphore
\item Buddy
\item LAVA
\item Buildbot
\item Opentest
\item Gentoo CI system
\item Fuego
\item 점검 툴을 자체 개발하여 사용중임. 
\item 사용안함
\end{enumerate}



5. pull request 1건당 최초의 코드리뷰를 받기 위하여 걸리시는 시간이 몇분인가요? 

\begin{enumerate}
\item 1분 이내 
\item 10분 이내
\item 30분 이내
\item 60분 이내 
\item 2시간 이내
\item 3시간 이내
\item 1일 이내 
\item 3일 이내
\item 6일 이내
\item 15일 이내
\item 30일 이내
\end{enumerate}



6. 당신은 다른 개발자가 제출한 pull reqeust를 코드 리뷰하기 위하여 얼마의 시간을 사용 하나요/

\begin{enumerate}
\item 1분 이내 
\item 10분 이내
\item 30분 이내
\item  60분 이내 
\item  2시간 이내
\item  3시간 이내
\item  1일 이내 
\item  3일 이내
\item  6일 이내
\item  15일 이내
\item  30일 이내
\item  기타 
\end{enumerate}
 



7. code review를 통해 실제 자신의 코드가 수정되는 빈도는 얼마나 됩니까?
 
\begin{enumerate}
\item 매우 잦음
\item 잦음
\item 보통
\item 거의 없음
\item 없음
\end{enumerate}




8. 개발 local PC에서 build 테스트후에 "git push"명령으로 pull request를 제출하나요?

\begin{enumerate}
\item 자체 빌드 테스트를 한후에 pull request를 제출한다. 
\item 나의 능력을 믿기 때문에 자체 빌드 테스트 없이 pull request를 제출한다. 
\item pull request를 제출하면 CI시스템이 자동으로 빌드를 테스트하기 때문에 굳이 자체 빌드 테스트를 수행하지 않는다. 
\item "git push" 명령이 무엇인지 모른다. 
\item 기타  
\end{enumerate}



9. 지금 개발중인 프로젝트에 pull request 마다 평균적으로 몇명이 코드리뷰를 참여  하고있나요? 

\begin{enumerate}
\item 0명
\item 1명
\item 2명
\item 3명
\item 4명
\item 5명+
\item 10명+
\item 50명+
\end{enumerate}



10.  개발중인 git repository에 pull request가 하루에 평균 몇 건정도가 올라오나요 ?

\begin{enumerate}
\item 0
\item 1+
\item 5+
\item 10+
\item 20+
\item 30+
\item 40+
\item 50+
\item 100+
\end{enumerate}


11. 제출하신 pull request가 merge 된 이후에는 몇 개의 OS/Platform을 대상으로 배포(deployment)가 진행됩니까?
1) 소스 코드 형태 (따로 배포되지 않음)
2) 1
3) 2
4) 3
5) 4+

12. 만약 배포가 이루어지고 있다면 어떤 OS/Platform을 대상으로 합니까? (중복 선택 가능)
1) Bianry Only (.out/.so/.exe 등)
2) RHEL/CentOS (.rpm 등)
3) Ubuntu/Debian (.deb 등)
4) Android (.apk 등)
5) Mac OS X (.pkg 등)
6) Windows (.msi 등)
7) 기타 


13 Reviewer의 리뷰코멘트를 통해 기술 역량을 향상시키는데 도움이 되고 있는가? 

\begin{enumerate}
\item 상당히 많이 되고있다. 
\item 많이 되고 있다. 
\item 도움이 되고 있다. 
\item 안하는것보다는 낫다. 
\item 도움이 안된다. 
\item 오히려 방해된다. 
\end{enumerate}


14. 당신이 생각하는 좋은 리뷰어란 어떤 사람인가요?
1. 코드의 실수를 조언하는 사람
2. 코드의 개선방향을 조언해주는 사람
3. 더 좋은  코드를 새로 아예 작성해주는 사람
4. 잘못된 코드부분을 꾸중해주는 사람
5. 가능한 변경한 코드 부분에 대해 모두 하나하나 일일이 물어보는 사람
6. 기타

15. 코드리뷰 필수화가 당사 제품의 소프트웨어 경쟁력에 관련이 있다고 보는가?
1. 코드리뷰는 반드시 해야 한다. 
1. 코드리뷰는 가능하면 하도록 권장해야 한다. 
1. 코드리뷰는 옵션이다. 
1. 코드리뷰가 소프트웨어 코드 품질에 영향을 미치지 않는다. 
1. 회사가 소프트웨어 회사이라면 코드리뷰같은것은 필요가 없다. 









이상. 

==> section/065_lesson_learned.tex <==

% Ref: 2019 FSE papers 
% Evaluating Model Testing and Model Checking for Finding, Requirements Violations in Simulink Models

This section describes the lessons we learned while running the proposed system on the public cloud, AWS case, using the new CI modules.

% \textbf{Handle Unstable CI Modules}. Sufficient aging tests are usually required before introducing new CI modules to avoid interruption to the continued operation of CI services and collaborative developments. At this time, even if the new CI feature test was completed on the local PC, there were times when the server did not operate normally due to an issue that was not found. We developed a CI retrigger called ``\textit{open sesame}'' to eliminate the latency of their PR inspections due to an error of a new CI feature. When developers add ``\textit{@open sesame m/d h:m}'' behind their PR title, the CI automatically re-runs. A responsive interface between developers and CI features enabled developers to respond to transient CI errors quickly.

\textbf{Lesson 1: Handle Unstable CI Modules}. Sufficient aging tests are usually required before introducing new CI modules to avoid interruption to the continued operation of CI services and collaborative developments. At this time, even if the new CI feature test was completed on the local PC, the server sometimes did not operate normally due to an issue that was not found. We developed a CI retrigger called ``\textit{open sesame}'' to eliminate the latency of their PR inspections due to an error of a new CI feature. When developers add ``\textit{@open sesame m/d h:m}'' behind their PR title, the CI automatically re-runs. A responsive interface between developers and CI features enabled developers to respond to transient CI errors quickly.


% \textbf{Plug-in Store to Encourage Participation}. Our plug-in architecture ensures easy addition and removal of module operations. We have developed a plug-in store prototype using \textit{modulator} to further enhance the functionality of the CI by encouraging the development of many external developers. Developers can register their modules in one of three categories: \textit{base}, \textit{good}, and \textit{staging}. When developers request registration after developing a new module, they can be added to the appropriate category through code reviews and aging tests. The registered modules can be added or removed in real-time during the operation of the CI system, making it easy for users to remove them via configuration easily.


\textbf{Lesson 2: Plug-in Store to Encourage Participation}. Our plug-in architecture ensures easy addition and removal of module operations. We developed a plug-in store prototype using the \textit{Modulator} to further enhance the functionality of the CI by encouraging the development of many external developers. Developers can register their modules in one of three categories: \textit{base}, \textit{good}, and \textit{staging}. When developers request registration after developing a new module, they can be added to the appropriate category through code reviews and aging tests. The registered modules can be added or removed in real-time during the operation of the CI system, making it easy for users to remove them easily via configuration.



% \textbf{Frequent PR Hangs with AWS Instances}. Public cloud services, such as AWS, allow creating server instances easily in a short time. Such services typically generate virtual machine (VM) instances as user machines, which may suffer from performance degradation due to the virtualization itself. From our experiments with Amazon AWS (e.g., m4.xlarge type, 4 vCPUs, 16 GB Memory), read throughput of AWS-HDD/st1 is 3 MB/s and that of AWS-SSD/gp2 is 250 MB/s. We compared the difference in reading and writing speed between two AWS storages in real-time using \textit{iotop} utility. The I/O speed of the AWS-HDD storage affects up to twelve times a build time of source code compared with the AWS-SSD/gp2. As a result, when many PRs are suddenly submitted, the slow I/O rate frequently causes an unintentional PR hang phenomenon temporarily.


\textbf{Lesson 3: Frequent PR Hangs with AWS Instances}. Public cloud services, such as AWS, allow server instances to be created quickly. Such services typically generate virtual machine (VM) instances as user machines, which may suffer from performance degradation due to the virtualization itself. From our experiments with Amazon AWS (e.g., m4.xlarge type, 4 vCPUs, 16 GB Memory), the read throughput of AWS-HDD/stl is 3 MB/s and that of AWS- SSD/gp2 is 250 MB/s. We compared the difference in reading and writing speed between two AWS storages in real-time using the \textit{iotop} utility. The I/O speed of the AWS-HDD storage affects the build time of source code up to twelve times that of the AWS-SSD/gp2. As a result, when many PRs are suddenly submitted, the slow I/O rate frequently causes an unintentional and temporary PR hang phenomenon.



% \textbf{Manage Unstable AWS Instance}. While running a CI server in AWS, we sometimes encountered instability in the AWS instance due to bugs of the Linux kernel, slow service, and system hanging. At this time, we introduced a function that CI manager restarts all services through a facility called ``\textit{Broken Arrow}'' (Fig. \ref{fig:pr-state-transition}) based on the web interface. This feature helps a CI administrator to eliminates an error of CI functionality due to an unstable AWS instance.


\textbf{Lesson 4: Manage Unstable AWS Instance}. While running a CI server in AWS, we sometimes encountered instability in the AWS instance due to bugs of the Linux kernel, slow service, and system hanging. At this time, we introduced a function enabling the CI manager to restart all services through a facility called ``\textit{Broken Arrow}'' (Fig. \ref{fig:pr-state-transition}) based on the web interface. This feature helps a CI administrator to eliminate an error of CI functionality due to an unstable AWS instance.


% \subsection{Running QEMU/ARM Emulator on AWS instance}\label{S_casestudy_aws_qemu_arm}
% X86 Ubuntu Developers use the QEMU-based software emulator technology when they need to run the Android emulator on their AWS instance to run the application's run test. However, the VM instance in AWS is a virtualization-based guest OS. Therefore, the VM instance cannot run the Android emulator because it does not have a virtualization instruction. We were able to run the QEMU ARM emulator in a virtualized guest OS by running an AWS instance using an x86 CPU architecture that supports \textit{nested virtualization} to properly run the QEMU-based Android emulator in the VM instance. This is because nested virtualization supports the \textit{vmx} virtualization instructions.


% Plan: let's omit this paragraph due to max 10 pages.
%\subsection{Build time of massive software}
% Massive open software projects such as \textit{Chromium}, \textit{PCL}, and \textit{TensorFlow} take 30 minutes or more to compile the source code. It means that the minimum amount of time a developer has to wait to check PR is 30 minutes or more. When building software with a long build time, building only the changed .so files can minimize the developer's wait time. Also, minimizing compilation range of the source code by using the latest-snapshot based prebuilt \textit{.so} files optimizes system resources.


==> trash/000_my_template.tex <==
% for proper tt fonts
\usepackage{fancyvrb}
\RecustomVerbatimEnvironment{verbatim}{Verbatim}{fontsize=\small}

\usepackage{letltxmacro}
% https://tex.stackexchange.com/q/88001/5764
\LetLtxMacro\oldttfamily\ttfamily
\DeclareRobustCommand{\ttfamily}{\oldttfamily\csname ttsize\endcsname}
\newcommand{\setttsize}[1]{\def\ttsize{#1}}%
\setttsize{\small}



% Enable line breaks with URL
\def\UrlBreaks{\do\/\do-\do.}

% Try to avoid overfull hbox
\setlength{\emergencystretch}{3pt}


% To display the page number at the bottom of each page 
\pagestyle{plain}

% To use math symbols
\usepackage{amsmath,amssymb,amsfonts}
\usepackage{algorithmic}
\usepackage{graphicx}
\usepackage{textcomp}
\usepackage{xcolor}

% To support Korean language
\usepackage{kotex}

% Display date, hour, and minute to maintain the paper version.
% Append the below statement in the 'abstract' section.
% [Notice] This document was compiled on: \today\ at \currenttime. 
\usepackage[short,nodayofweek,level,24hr]{datetime}


% Text highlight and color (e.g. \hl, \textcolor )
\usepackage{xcolor,color,soul}
%\usepackage{soul}

% Hyperlinks to content
%\usepackage[linktocpage=true]{hyperref}
\usepackage{hyperref}
\hypersetup{
  colorlinks   = true, %Colours links instead of ugly boxes
  urlcolor     = blue, %Colour for external hyperlinks
  linkcolor    = black,  %Colour of internal links
  citecolor    = black  %Colour of citations, could be ``red''
}

% Hyperlinks to content
% 1. for IEEEtran.cls
% \usepackage[linktocpage=true]{}
% \usepackage[linktocpage=true,colorlinks=true,linkcolor=blue, citecolor=blue, urlcolor=blue]{hyperref}
%
% 2. for acmart.cls : acmart.pdf file --> page 8 --> Table 2: Boolean options
% - review: false(default), A review version: lines are numbered and hyperlinks are colored
% - screen: see text, A screen version: hyperlinks are colored
% - case study for acmart.cls: \documentclass[...,review, screen,...]{acmart}


% for using a number symbol (\ding{3})
\usepackage{pifont}




% How to support a code listing
\usepackage{listings}

% set the default code style
\lstset{
    frame=tb, % draw a frame at the top and bottom of the code block
    tabsize=4, % tab space width
    showstringspaces=false, % don't mark spaces in strings
    numbers=left, % display line numbers on the left
    commentstyle=\color{green}, % comment color
    keywordstyle=\color{blue}, % keyword color
    stringstyle=\color{red} % string color
}

% Table packages:
\usepackage{threeparttable}
\usepackage[table]{xcolor}
\usepackage{booktabs,tabulary}
\usepackage{siunitx}
\usepackage{float}
\usepackage{booktabs, makecell, tabularx,}
\renewcommand\theadfont{\bfseries}


%\usepackage{multirow}
%\setlist{nosep} % Reduce itemize/enumerate spaces
% \setlist[itemize,1]{leftmargin=\dimexpr 1.5em}
\setlist[enumerate,1]{leftmargin=\dimexpr 1.5em}

==> trash/archive/013_ccs.tex <==

%
% The code below should be generated by the tool at
% http://dl.acm.org/ccs.cfm (The ACM Computing Classification System (CCS))
% Please copy and paste the code instead of the example below.
%
\begin{CCSXML}
<ccs2012>
 <concept>
  <concept_id>10010520.10010553.10010562</concept_id>
  <concept_desc>Computer systems organization~Embedded systems</concept_desc>
  <concept_significance>500</concept_significance>
 </concept>
 <concept>
  <concept_id>10010520.10010553.10010562.10010564</concept_id>
  <concept_desc>Computer systems organization~Embedded software</concept_desc>
  <concept_significance>500</concept_significance>
 </concept>
 <concept>
  <concept_id>10011007.10011074.10011099</concept_id>
  <concept_desc>Software and its engineering~Software verification and validation</concept_desc>
  <concept_significance>500</concept_significance>
 </concept>
 <concept>
  <concept_id>10011007.10011074.10011134</concept_id>
  <concept_desc>Software and its engineering~Collaboration in software development</concept_desc>
  <concept_significance>500</concept_significance>
 </concept>
</ccs2012>
\end{CCSXML}

\ccsdesc[500]{Computer systems organization~Embedded systems}
\ccsdesc[500]{Computer systems organization~Embedded software}
\ccsdesc[500]{Software and its engineering~Software verification and validation}
\ccsdesc[500]{Software and its engineering~Collaboration in software development}

==> trash/archive/020_introduction_00.tex <==

 Recently, the computing environment has evolved from cloud computing to edge computing. In edge computing, Internet-of-Things (IoT) devices store the collected data on the cloud computer in real time. Many existing devices are equipped with connectivity such as the internet. As a result, various IoT devices with different hardware structures have been increasing exponentially.

Such IoT devices usually operate continuously 24/7. To guarantee uninterrupted service, such devices have to be updated frequently and automatically\textemdash we cannot afford manually updating IoT devices or delaying updates for a long time\textemdash to help prevent potential security defect, performance deterioration, or behavioral issues in run time.

The complexity of software is becoming higher even for lightweight IoT devices. With such a complexity, a software update incurred by a code commit is required to be integrated to deployed system \cite{6448697} in real time in order to reduce the latency, which is critical to the security and overall system robustness: we may want every node to share the same recent versions. Therefore, the software integration \cite{6802994} and deployment latency from the code commit is emerging as a key pain point for software platform deployment.

 최근에 중앙 서버와 네트워크를 통해 IoT 디바이스와 통신하는 클라우드 컴퓨팅은 아래와 같이 3가지의 새로운 문제에 직면하고 있다. 
\begin{itemize}
\item 서비스 제공 지연 문제: 실시간 서비스 제공이 어려워지고 있다. 
\item 처리 부하 및 비용증가: 클라우드와 연계하는 IoT 기기의 수가 급격히 증가하고 있다. 시장조사기관 가트너 통계에 의하면, IoT 기기수는 2020년 300억개에서 2025년에 750억개로 증가할것으로 전망하고 있다. \cite{statista-iot-number}
\item 정보 침해성: 중요 정보를 클라우드 제공자에게 맡기기 어려운 이슈를 가지고 있다. 
 \end{itemize}
 
 이로 인해 기존의 클라우드 컴퓨팅 구조의 단점을 보완하기 위하여 엣지 컴퓨팅이 대두되고 있다. 최근에 엣지 기기 자체의 컴퓨팅 파워 증가로 인하여 과거에는 단순이 데이터를 수집하고 전송하는 역할만 수행하였으나 최근에는 일부 데이타를 연산처리하는 기능도 수행하고 있다. IoT 기기와 엣지 디바이스들의 폭발적인 증가로 인해 현재보다 더 많은 상이한 소프트웨어 플랫폼 이미지들이 더 주기적으로 피쳐 추가 및 보안 픽스를 위하여 현재보다 플랫폼 이미지의 업데이트 주기가 증가할수 밖에 없다. 이러한 환경에서 소프트웨어 플래폼 이미지의 주기적인 업데이트가 안정적으로 보장되기 위하여 소프트웨어의 지속적인 통합을 저해하는 요소를 해결하는 기술은 매우 중요하다. 

GitHub.com은\cite{Kalliamvakou:2014:PPM:2597073.2597074} 소스코드들이 충분한 리뷰와 코드의 테스트들을 수행함으로써 추가로 유입되는 소스코드들의 취약성이 소프트웨어의 안정성과 기능성을 훼손 시키는 문제를 방지한다. 특히, GitHub.com의 Pull Request (PR)는 기존의 소스 코드 제어 시스템들이 다루지 못하였던 코드 리뷰 절차를 통한 코드의 병합 시스템을 제공한다. 

그러나 이러한 서비스 들은 CI의 기능성보다 인프라스트력처에 집중을 하고 있기 때문에 많은 개발자들이 Pull Request (PR)의 장점을 실제로 활용하지 못하는 경우가 빈번하다. 

그 결과 대표적인 오픈소스 프로젝트 외에 대부분의  소프트웨어 프로젝트 들이 충분한 코드리뷰와 검사 절차 없이 코드의 병합이 이루어 지고 있다. 또한 종종 소스 코드의  자체 빌드 검사를 수행하지 않고 직접 코드를 병합하여 같이 개발하는 다른 개발자들의 소스코드 빌드 및 실행 테스트를 방해하고 있다. 

소프트웨어 개발 시 코드 품질을 향상시키기 위하여 코드를 점검 하기 위한 리뷰 프로세스 및 리뷰 문화는 지속적으로 문제가 되어 왔다. 제안하는 시스템은  자동화된 시스템이 코드리뷰 업무를 자동화하고 미리 코드에 대한 평가를 하여 리뷰어가 보다 핵심적인 내용에 집중하도록 한다. 그 결과 리뷰의 질과 속도를 높이고 기존 업무의 비효율적 요소들을 제거한다. 

 
리뷰어가 많은 시간과 노력을 들여서 모든 종류의 소스코드 내 결함들을 직접 개별 확인해야 하여 리뷰어들이 리뷰를 소흘히 하거나 리뷰에 지나치게 많은 시간이 소모되는 업무 비효율성이 있다.  그 결과 많은 프로젝트들의 소프트웨어 개발 경쟁력이 퇴보하는 악순환이 반복되어 소프트웨어 완성도에 막대한 손실을 가져다 주고 있다. 


개발자들이 소프트웨어 코드를 작성할 때마다 리뷰어들이 자발적으로 코드를 리뷰하고 있습니다. 그 결과 개발자들이 리뷰에 참여하는 시간이 증가할수록 본연의 업무에 집중할 수 있는 시간이 줄어드는 문제를 야기하고 있다. 그리고, 소프트웨어 코드를 리뷰 하는 것은 자발적 업무에 해당하기 때문에 코드리뷰에 자신의 업무 시간을 많이 할애하지 않는 성향을 가진다. 그 결과 코드 리뷰가 부실하거나 유명무실한 리뷰만으로 소프트웨어를 개발하는 과제들이 빈번히 발생하고 있다. 

자동화된 시스템을 통하여 미리 잘못 작성된 코드를 거절하여 리뷰어가 점검해야 하는 코드의 양을 줄일수 있다. 리뷰어가 점검해야 할 항목들을 줄임으로써 리뷰어는 생산적인 코드 리뷰에 집중할수 있다. 리뷰어가 코드의 품질을 높이는데 집중할수 있음으로써 소프트웨어의 전반적인 개발 효율성 향상시킬수 있다.


우리의 설문 조사결과 개발자들이 상품화 프로젝트를 진행할때, 10명 이내의 개발자들이 소스들을 협업 개발시에 다른 개발자들이 제출한 Pull Request에 대한 코드의 전문성을 가지고 있지 않는 경우가 많다. 뿐만 아니라 개발자가 소프트웨어 릴리즈 일정을 준수하기 위하여 자신의 모듈 개발에 집중하여야 하는 상황일때 다른 개발자들이 개발중인 코드  리뷰를 참여할 시간적인 여유가 없는경우가 빈번하다. 실제의 기업 개발환경에서 코드의 취약성은 코드가 결합되기 이전에 충분한 점검을 수행하지 않기 때문에 소프트웨어의 릴리즈 시점에 이러한 잘못된  소프트웨어 결함 수정에 개발시간을 많이 빼아긴다. 그 결과 소프트웨어의 릴리즈 일정을 지연시키는 결과를 초래한다. 


사회 전반에 소프트웨어를 이용한 사회 구축 시스템이 활발히 진행되고 있다. 결함을 가진 소프트웨어 코드가 기존 소스코드에 병합이 되었을때 소프트웨어 기반의 사회 전산 시스템은 엄청난 비용과 당초의 사업일정을 지연시킨다. 최근에  Obamacare  웹사이트에서 2천만명의 미국인들이 서비스 시작후 로그인 자체가 안되는 소프트웨어 사고가 있었습니다. Obamacare 는 가족 구성원들이 보험에 가입하도록 돕고 건강을 지킬수 있도록 하기위한 사회 시스템이다. Obamacare 서비스는 충분한 코드 결함 점검과 코드리뷰를 수행하지 않고 소프트웨어 출시 일정에 집중한 결과 아래와 같은 소프트웨어 결함들이 잠재하고 있었다. 

\begin{itemize}
\item 웹사이트가 너무 많은 'cookie' 추적 데이타를 작성하여 로그인 정보를 수용할수 있는 사이트 용량을 초과하였다. 
\item 2가지 보안 취약점을 이용하여 사용자 계정을 도용할수 있었다. 
\begin{itemize}
\item 사이트의 오류메세지가 암호화 없이 인터넷을 통해 개인정보를 전달하였다. 
\item 전자 메일 확인 시스템은 전자 메일계정에 엑세스하지 않고 우회가 가능하였다. 
\end{itemize}
\item 사이트의 기본 아키텍쳐는 설계에 결함이 있었고, 제대로 테스트를 수행을 하지 않았다. 
\item 사이트의 백엔드에서도 데이타가 왜곡 되어 일부 경우에 데이타를 사용 할수 없게 되었다. 
\end{itemize}

우리는 소프트웨어 플랫폼을 릴리즈하기 위하여 필요한 패키지들을 협업 개발중에 많은 소프트웨어 취약성들이 잘못된 프로그래밍의 반복된 실수들로 인하여 취약성 똰 반복하여 이러 난다는 사실을 관찰할수 있다. 이러한 문제는 리뷰어 들이 코드의 리뷰 시간을 생산적으로 사용하지 못하는 결과를 만든다. 우리는 본 논문에서 가볍고 확장가능한 자동화 리뷰어 시스템을 설계하고 구현함으로써 지속적인 코드의 결합이 제공할수 있는 방법들을 상세히 소개한다. 

Especially, users continuously require new features of the software and there are large software packages with more than hundreds of actively participating developers in a single software package such as \textit{Caffe}, and \textit{Tensorflow} in case of Edge Artificial Intelligence (AI). The more size of software gets bigger and complicated, the more we need to inspect the code and prevent errors from new code commits before deployment especially if we have a lot of devices deployed with diversities in their architectures and hardware configurations; more devices mean more potential failures. \cite{6606557} Therefore, the integration, deployment latencies \cite{Waller:2015:IPB:2735399.2735416}, and the error prevention capabilities of CI systems \cite{6802994} are critical.

이 논문에서의 제안하는 우리의 시스템이 제공하는 주요 contribution은 다음과 같다. 
\begin{itemize}
    \item Resource-aware lightweight system: 기존의 대부분의 CI 시스템들은 고사양의 하드웨어 스펙을 필요로 한다. 기존 시스템들은 CI의 인프라스트럭쳐에 집중을 하고있다. 그러나 우리의 제안 시스템은 CI의 기능성에 집중한다. 우리는 최신으로 설계된 webhook event기반의 핸들러와 PR들의 테스트 자동화 와 결함 점검기능에 집중한 재조립 가능하고 확장가능하며 일반적인 desktop pc에서도 운영가능한 가볍고 빠른 시스템을 제안한다.  
    \item Unified source code manager (caching, one clone): 우리는 체커들이 수행할때마다 반복적으로 수행하는 동일한 소스코드의 다운로를 제어하기 위하여 Pull request가 제출되었을때 모든 체커들이 공유하여 사용가능한 변경된 소스코들을 관리하는 git clone accelerator을 제공한다. Wehhook handler가 이 기능을 담당한다. 
    \item Out-of-PR Killer: 개발자가 소스 코드를 작성하여 PR을 제출후에 잘못작성한 코드를 수정하여 다시 PR을 제출할때마다 CI서버는 중복된 PR을 작업을 기본적을 수행한다. 개발자가 새로수정한 동일한 PR을 제출할때 제안 시스템은 LRU 알고리즘에 기반하여 이전에 실행중인 동일한 PR의 작업을 killing하는 기능을 제공한다. 릴리즈 일정이 도래하였을때 이러한 중복된 PR의 수가 항상 증가하고, 그 결과 OOP Killer가 없는 시스템는 자동화 시스템의 실행속도가 지연되어 코드의 병합이 지연되는 결과를 초래한다. 
    \item Plug-in Store: 개발 프로젝트마다 동일한 기능을 수행하는 공통의 모듈들이 있다. 반면에 각각의 프로젝트마다 코드를 점검하기 위한 다른 모듈들이 있다. 개발자는 기존의 모듈들을 플러그인 구조를 이용하여 쉽게 코드의 장애 없이 추가 또는 해제할수 있다. 뿐만 아니라 각각의 개발 프로젝트를 위해 필요한 모듈들을 플러그인 구조로 유연하게 추가하여 점검 기능을 강화할수 있다.  플러그인들은 그 기능성과 안정성의 정도에 따라 base, good, staging으로 분리된다. 
    \item Fine-grained inspector (before build, after build): 제안 시스템은 코드의 점검 자동화를 빌드전과 빌드후의 2가지의 카테고리로 분류한다. 수십명의 개발자들이 소스코드를 개발하면서 대부분의 소프트웨어 결함이 빌드전에 발견될수 있고, 빌드전에 발견되는 결함들은 빌드과정을 진행하지 않음으로써 소프트웨어 코드의 빌드시에 발생하는 비용을 최소화할수 있다. 제안시스템은 빌드전의 format checker와 빌드후의 audit checker으로 분류한다. 
    \item Portability: 기존의 CI 기법들은 개발자들이 다른 프로젝트에 기존의 CI 기능등을 재사용하려고 할 경우에 기존 시스템의 설계는 이식성을 고려하지 않았기때문에 추가적인 비용이 많이 필요하다. 제안 아이디어는 플러그인 방식으로  CI 기능들을 착탈식으로 사용가능하다. 기존의 CI 솔류션들은 개발자들이 추가 모듈을 개발하기 위하여 새로운 작성 규칙의 문법구조와 많은 API들을 사용해야 한다. 그러나 우리 솔류션은 4개의 API만으로 대부분의 개발자들이 익숙한 Shell script 문법구조로 필요한 추가 모듈을 쉽게 확장가능하다. 
\end{itemize}
  
The reminder of the paper is organized as follows. The build time of modern software is described in Section II. Section III addresses the design and implementation of the proposed techniques in detail. Section IV shows the evaluation results, and related work is described in Section V. Finally, Section VI concludes the paper.
